Breaking the Benchmark: Revealing LLM Bias via Minimal Contextual Augmentation

Large Language Models have been shown to demonstrate stereotypical biases in their representations and behavior due to the discriminative nature of the data that they have been trained on. Despite significant progress in the development of methods and models that refrain from using stereotypical information in their decision-making, recent work has shown that approaches used for bias alignment are brittle. In this work, we introduce a novel and general augmentation framework that involves three plug-and-play steps and is applicable to a number of fairness evaluation benchmarks. Through application of augmentation to a fairness evaluation dataset (Bias Benchmark for Question Answering (BBQ)), we find that Large Language Models (LLMs), including state-of-the-art open and closed weight models, are susceptible to perturbations to their inputs, showcasing a higher likelihood to behave stereotypically. Furthermore, we find that such models are more likely to have biased behavior in cases where the target demographic belongs to a community less studied by the literature, underlining the need to expand the fairness and safety research to include more diverse communities.

==> motivating_studies_from_social_science.tex <==
\section{Motivating Studies from Social Science}

%Beyond the well-known biases that have been widely studied in prior NLP literature, social scientists have found that people are prone to a slew of subtler biases based on traits often assumed to be relatively innocuous. These traits include beauty, age, associated institution, and nationality.

%\citet{dion1972beautiful} studied how attractiveness is related to socially desirable occupational status, personal traits, etc. They found that people who are considered attractive are more likely to hold socially desirable traits.

\citet{dion1972beautiful} found that people who are considered attractive are more likely to believed to hold socially desirable traits and higher occupational status. \citet{gross1977good} found that such biases also occur in the opposite direction---that knowing that people have desirable qualities lead us to judge them as more beautiful. Attractiveness plays a measurable role in employee termination \cite{commisso2012physical}, hiring processes \cite{marlowe1996gender}, interview callbacks \cite{maurer2015rare}, and even in victim blaming \cite{weber2013blaming}.

%\gknote{We should reword to as ``more likely to hold socially desirable traits''. Just saying that they are more socially desireable makes it sound like we're just saying people like physically attractive people, not that people infer additional characteristics about them.}. 
%They also found that attractiveness is a major factor in judging people's occupations. %and this finding inspires us to add professions in our beauty attribute section.
%\gknote{We should move the study design details for later. We can refer back to this paper when we describe the design. But it's cluttered to jump the gun and start discussing that now.}
%\citet{gross1977good} conducted an experiment in the reverse direction to \citet{dion1972beautiful} and found that knowing that people have good qualities affects our judgments of how beautiful we find them to be. 
%These two studies \cite{dion1972beautiful, gross1977good} motivated us to design our work in two directions i.e., Stimulus to Attribute Inference (SAI) and Attribute to Stimulus Association (ASA).\gknote{Same issue as above. We should move the discussion of study details later.} 
%Also, attractiveness plays a measurable role in employee termination \cite{commisso2012physical}, hiring processes \cite{marlowe1996gender}, interview callbacks \cite{maurer2015rare}, and even in victim blaming \cite{weber2013blaming}. As LLMs are widely used nowadays, we must address the degree to which such beauty bias is present in large language models. 

\citet{perdue1990evidence}, \citet{axelrod1961attitudes}, and \citet{aaronson1966personality} found that people are more likely to infer negative traits and stereotypes on people that are older or labeled as ``old'' as opposed to ``young''. This validates \citeposs{butler1969age} earlier introduction of the term ``ageism'', referring to discrimination towards elderly people. As with beauty, age has been found to be a factor in evaluating workers~\cite{ng2012evaluating}.
%, where typically older workers are wrongly evaluated as worse~\cite{ng2012evaluating}.


%\citet{butler1969age} introduced the term ``agesim'' which refers discrimination towards elderly people. \citet{perdue1990evidence} studied how social category labels such as ``old'' and ``young'' influence the inferred positive and negative traits in the same people. From their study, they found that negative traits are most likely related to aged people. \citet{axelrod1961attitudes} also found that negative stereotypes increased with age. 
%From \citet{aaronson1966personality}'s study, it is clear that personal trait assumptions are closely related to age.
%\citet{aaronson1966personality} confirmed \citeauthor{axelrod1961attitudes}'s~(\citeyear{axelrod1961attitudes}) results, making it clear that personal trait assumptions are strongly associated to age. 
%\gknote{why is there only one citation when the sentence refers to ``different studies''?}. 
%As with beauty, age has also been found to be a factor in evaluating workers, where typically older workers are wrongly evaluated as worse~\cite{ng2012evaluating}.

Organizations and institutions have been found to be associated with specific personality traits, both within the US~\cite{slaughter2004personality} and internationally~\cite{anderson2010personality}. \citet{rutter2017brand} found that universities leverage specific personality traits when branding and \citet{humburg2017personality} student personality traits play an important role in student choice of university and alternatives (e.g., vocational education). Such bidirectional effects of personality traits result in hiring biases that prioritize students from academic institutions with particular reputations~\cite{morley2007employers,mavridopoulou2020elitism}.

%\citet{slaughter2004personality} studied how personality traits are related to an organization or institution. In their experiment, they used different organizations (e.g., Microsoft, Nike, Walmart, etc.) and investigated how personal traits differ in these organizations.
%\gknote{What were the major findings? What type of relationship between major organizations and personality traits did they find?} 
%While this study was limited to the US, \citet{anderson2010personality} performed an extended global study and included more organizations. 
%While this study focuses on general institutions, other studies focus on educational institutions. 
%Along these lines, the reputation of an academic institution plays an important role in alumni hiring and in many cases recruiters prioritize students from elite institutions~\cite{morley2007employers, mavridopoulou2020elitism}. In his study, \citet{humburg2017personality} found that personality traits also play an important role in student choice of university and other institutions (e.g., vocational education). Top universities leverage specific personality traits when branding, which may be one of the factors behind why people assume that students from higher-ranked universities possess a broad range of positive personality traits compared to others~\cite{rutter2017brand}.

%Racial behaviors developed among people from their childhood and eventually resulted in intergroup bias (e.g., nationality bias) \cite{monteiro2009development}.\gknote{This sentence suggests that racial bias would be more appropriate. We should rephrase this or move it later so that we can motivate our choice of bias better.} Nationality bias affects various aspects of our life.\gknote{I don't see the purpose of this sentence.} 

Nationality bias has found to affect student interactions in multicultural online learning environments~\cite{morales2020nationality}, consumer perception towards products~\cite{insch2004impact}, academic philosophy~\cite{seabra2023cognitive}, and peer evaluation~\cite{tavoletti2022nationality}. \citet{tavoletti2022nationality} identified the economic development of a person's country of origin as an important factor within this bias, overshadowing individual qualities when one evaluates their peers.

As LLMs are trained on data created by humans, we hypothesize that they are prone to similar biases to those identified in people. If present, we must measure the degree to which such biases are present so that we can appropriately account for them when LLMs are used for consequential decisions, such as recruiting and hiring.

%Nationality plays an important role in multicultural online learning environments which has been found to affect student interactions~\cite{morales2020nationality}, consumer perception towards products~\cite{insch2004impact}, and academic philosophy~\cite{seabra2023cognitive}.
%\gknote{What kind of important role? This sentence is too vague/generic to be useful.}  
%\citet{tavoletti2022nationality} studied how nationality bias affects peer evaluation. They found that the nationalities of team members is a real, potential source of bias in peer evaluation. They further found that the economic development level of the team member's country of origin is seen as an important factor in evaluating peers over their individual qualities. 
%They use economic conditions (GDP per capita) to categorize countries, and we motivated from this study to use GDP per capita in our study.\gknote{Same issue as in the beauty bias section. Our study design details should come later. We can refer to this paper there as our motivation.}

==> tables/Phi4_Secondary.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{c lcc}
\hline
\textbf{\rotatebox{90}{}} & \textbf{Type} & \textbf{Not taking a definite side (\%)} & \textbf{Taking a definite side (\%)} \\
\hline
\multirow{15}{*}{\rotatebox{90}{More Studied}} 
& original\_context\_original\_question & 98.41 & 1.59 \\
& augmented\_scenarios\_original\_question & 91.41 & 8.58 \\
& augmented\_scenarios\_question2 & 85.18 & 14.81 \\
& augmented\_scenarios\_question3 & 89.06 & 10.93 \\
\hline
\multirow{15}{*}{\rotatebox{90}{Less Studied}} 
& original\_context\_original\_question & 96.50 & 3.50 \\
& augmented\_scenarios\_original\_question & 88.19 & 11.80 \\
& augmented\_scenarios\_question2 & 81.68 & 18.31 \\
& augmented\_scenarios\_question3 & 84.08 & 15.91 \\
\hline
\end{tabular}
\caption{Percentage of responses for each question type, grouped by More studied vs. Less studied for \textbf{Phi4-14B}, comparing those not taking a definite side versus those taking a definite side.}
\label{tab:definite_side_percent_with_group_deepseek}
\end{table*}

==> tables/gemini.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{c lcc}
\hline
\textbf{\rotatebox{90}{}} & \textbf{Type} & \textbf{Not taking a definite side (\%)} & \textbf{Taking a definite side (\%)} \\
\hline
\multirow{4}{*}{\rotatebox{90}{More}} 
& original\_context\_original\_question & 94.46 & 5.54 \\
& augmented\_scenarios\_original\_question & 86.20 & 13.79 \\
& augmented\_scenarios\_question2 & 81.84 & 18.15 \\
& augmented\_scenarios\_question3 & 90.54 & 9.45 \\
\hline
\multirow{4}{*}{\rotatebox{90}{Less}} 
& original\_context\_original\_question & 91.53 & 8.47 \\
& augmented\_scenarios\_original\_question & 79.92 & 20.07 \\
& augmented\_scenarios\_question2 & 77.32 & 22.67 \\
& augmented\_scenarios\_question3 & 84.99 & 15.01 \\
\hline
\end{tabular}
\caption{Percentage of responses for each question type, grouped by More studied vs. Less studied for \textbf{Gemini-2.5-Flash-Lite}, comparing those not taking a definite side versus those taking a definite side.}
\label{tab:definite_side_percent_with_group_deepseek}
\end{table*}

==> tables/qwen3_14b.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{c lcc}
\hline
\textbf{\rotatebox{90}{}} & \textbf{Type} & \textbf{Not taking a definite side (\%)} & \textbf{Taking a definite side (\%)} \\
\hline
\multirow{4}{*}{\rotatebox{90}{More}} 
& original\_context\_original\_question & 91.95 & 8.05 \\
& augmented\_scenarios\_original\_question & 79.92 & 20.07 \\
& augmented\_scenarios\_question2 & 73.96 & 26.30 \\
& augmented\_scenarios\_question3 & 86.60 & 13.39 \\
\hline
\multirow{4}{*}{\rotatebox{90}{Less}} 
& original\_context\_original\_question & 84.74 & 15.26 \\
& augmented\_scenarios\_original\_question & 79.49 & 26.50 \\
& augmented\_scenarios\_question2 & 66.36 & 33.63 \\
& augmented\_scenarios\_question3 & 76.47 & 23.52 \\
\hline
\end{tabular}
\caption{Percentage of responses for each question type, grouped by More studied vs. Less studied for \textbf{Qwem3-14B}, comparing those not taking a definite side versus those taking a definite side.}
\label{tab:definite_side_percent_with_group_deepseek}
\end{table*}

==> tables/qwen3_4b.tex <==
\begin{table*}[htbp]
\centering
\small
\begin{tabular}{c lcc}
\hline
\textbf{\rotatebox{90}{}} & \textbf{Type} & \textbf{Not taking a definite side (\%)} & \textbf{Taking a definite side (\%)} \\
\hline
\multirow{4}{*}{\rotatebox{90}{More}} 
& original\_context\_original\_question & 66.95 & 33.05 \\
& augmented\_scenarios\_original\_question & 86.03 & 13.96 \\
& augmented\_scenarios\_question2 & 81.67 & 18.32 \\
& augmented\_scenarios\_question3 & 79.52 & 20.47 \\
\hline
\multirow{4}{*}{\rotatebox{90}{Less}} 
& original\_context\_original\_question & 52.85 & 47.15 \\
& augmented\_scenarios\_original\_question & 81.68 & 18.31 \\
& augmented\_scenarios\_question2 & 77.97 & 22.02 \\
& augmented\_scenarios\_question3 & 65.29 & 34.70 \\
\hline
\end{tabular}
\caption{Percentage of responses for each question type, grouped by More studied vs. Less studied for \textbf{Qwem3-4B}, comparing those not taking a definite side versus those taking a definite side.}
\label{tab:definite_side_percent_with_group_deepseek}
\end{table*}

==> task_definition.tex <==
\section{Task Definition}
%Following \citet{vinacke1957stereotypes, nadeem-etal-2021-stereoset, caliskan2017semantics}, we define stereotype as unfair and over-generalized beliefs about a group of people based on some particular facts\gknote{What do you mean by ``over-generalized beliefs about a group of people based on some particular facts''. This sentence doesn't seem to say anything to me.}.
%In this study, we assess bias in generative large language models. 
%In the previous studies of bias in LLMs, authors measured the presence of bias in one direction. 
Unlike previous studies which have focused on identifying bias in a single direction, we take a more general measurement by considering two directions of bias.
For example, \citet{nadeem-etal-2021-stereoset} measured stereotypes of LLMs by giving the \textit{race} description (e.g., Hispanic, Ghanaian etc.) or a \textit{profession} (e.g., physicist, tailor, etc.) and asked LLMs to choose between stereotypicallty associated \textit{attributes} (e.g., poor, creative, etc.), % stereotypically related to \textit{race} or \textit{profession}, 
but they did not measure the bias in reverse context (e.g., by giving \textit{attributes} and asking LLMs to choose the associated \textit{race} or \textit{profession}). In our study, we study both directions, inspired by \citeauthor{dion1972beautiful}'s~(\citeyear{dion1972beautiful}) and \citeauthor{gross1977good}'s~(\citeyear{gross1977good}) work showing that people demonstrate beauty bias in both directions. 
%\citeauthor{dion1972beautiful}'s~(\citeyear{dion1972beautiful}) work which found that attractiveness significantly affects judgments about individuals' socially desirable traits and occupational status, and \citeauthor{gross1977good}'s~(\citeyear{gross1977good}) which reversed this line of inquiry by showing that positive qualities or traits can affect our perception of someone's attractiveness, we aim to measure the bias in both directions. 
%we measured the bias in both directions, which ensures more generalizations\gknote{This motivation is too general. What are the specific motivations that the cited studies have for reversing the direction? Alternatively, what about those papers' conclusions warrant our reverse direction experiment?}. 
In our experiment, we use \textit{fill-in-the-blank} style sentences which evoke the biases in the provided text using a description of a person based on the bias category we are studying. We will refer to this description as simply the \textbf{\textit{stimulus}}. For example, in Figure~\ref{fig:example} (a), the stimulus is ``Hinds Community College'' for institutional bias.

We consider a system to be biased if the conditional likelihood of positive, negative, or neutral completions change when the polarity of the prompting text changes. That is, an unbiased system will have $\Delta$PL, $\Delta$NL, and $\Delta$NuL values~(defined in Figure~\ref{fig:delta-graph}) of 0. For example, in Figure~\ref{fig:delta-graph}, we find that $\Delta$NL is systematically negative, so the negative predictions of the models are biased in the opposite direction of the prompt text changes.
%Can we just say that if the $\Delta$ PL, NL or NuL is not zero then we can say that it is biased towards a particular side. Fore example, when $\Delta$ NL is not zero then there exits bias and as our cases the value of $\Delta$ NL is negative, we can say that it it biased towards negative}

\paragraph{Stimulus to Attribute Inference (SAI):} We provide %\gknote{Right now ``category'' is too vague. Perhaps we can write ``we provide a descriptor that evokes a biased category, which we will simply refer to as a \textit{category}''.} 
a \textit{stimulus} and ask the LLM to infer a related \textit{attribute}. The LLM must choose between a set of three attributes: positive, negative, and neutral. In Figure~\ref{fig:example} (a), the stimulus is ``Hinds Community College'' and positive, negative and neutral attributes are ``innovative'',``unimaginative'', and ``chummy'', respectively. 
%\gknote{We should have a running example, perhaps in a figure. We can refer to the example throughout the task definition to make it clear.}

\paragraph{Attribute to Stimulus Association (ASA):} We provide \textit{attribute} and ask the LLM to choose a specific \textit{stimulus}. The LLM must choose between a set of three stimuli: positive, negative, and neutral. In Figure~\ref{fig:example} (b), the attribute is ``energetic'' and the positive, negative and neutral stimuli are ``University of california, san diego'', ``Ivy tech community college'', and ``Wichita'' respectively.



%We also measure how LLMs respond in terms of positive and negative attributes.





\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{Merged.jpg}
\captionof{figure}{A high-level of diagram of our dataset sample creation procedure in both SAI and ASA directions. In the SAI direction, if we pick ``unattractive'' as a stimulus, then the examples will be ``He looks unattractive, he is BLANK'', ``She looks unattractive, she is BLANK'', ``They look unattractive, they are BLANK''; then we give 3 attributes as options to fill the BLANK. We also do this for all other stimuli for additional examples. In the ASA direction, if we pick ``smart'' as an attribute, then the examples will be ``He looks BLANK, he is smart'', ``She looks BLANK, she is smart'', ``They look BLANK, they are smart''; then we give 3 stimuli as options to fill the BLANK. We also do this for all others attributes.}
\label{fig:meth}
\end{figure*}
